Reward Machines: Exploiting Reward Function Structure in Reinforcement Learning

Reinforcement learning (RL) methods usually treat reward functions as black boxes. As such, these methods must extensively interact with the environment in order to discover rewards and optimal policies. In most RL applications, however, users have to program the reward function and, hence, there is the opportunity to make the reward function visible -- to show the reward function's code to the RL agent so it can exploit the function's internal structure to learn optimal policies in a more sample efficient manner. In this paper, we show how to accomplish this idea in two steps. First, we propose reward machines, a type of finite state machine that supports the specification of reward functions while exposing reward function structure. We then describe different methodologies to exploit this structure to support learning, including automated reward shaping, task decomposition, and counterfactual reasoning with off-policy learning. Experiments on tabular and continuous domains, across different tasks and RL agents, show the benefits of exploiting reward structure with respect to sample efficiency and the quality of resultant policies. Finally, by virtue of being a form of finite state machine, reward machines have the expressive power of a regular language and as such support loops, sequences and conditionals, as well as the expression of temporally extended properties typical of linear temporal logic and non-Markovian reward specification.

==> TODO.tex <==
TODO list for final version (if accepted)

\begin{itemize}
\item add acknowledgements
\item check how colors appear in black-and-white
\end{itemize}

==> src/learn.tex <==
\begin{algorithmic}[1]
    \STATE {\bfseries Input:} $\mathcal{P}$, $L$, $\gamma$, $\Sigma=[\ldots\tuple{U^{i},u^{i}_0,\delta^{i}_u,\delta^{i}_r}\ldots]$.
    \STATE $\Qapprox \leftarrow$ InitializeQValueFunctions($\Sigma$)
    \FOR{$l=0$ \TO num\_episodes} 
        \STATE $i \leftarrow$ GetTask($\Sigma$, $l$)%l\bmod|\Sigma|$ \COMMENT{\textit{Run an episode solving task $i$}}
        \STATE $u^{i}_p \leftarrow u^{i}_0$; $s \leftarrow$ EnvInitialState()
        %\WHILE{EnvDeadEnd($s$) $\neq$ True}
        \FOR{$t=0$ \TO length\_episode} 
            \IF{EnvDeadEnd($s$)} 
                \STATE \textbf{break}
            \ENDIF
            \STATE $a \leftarrow$ GetActionEpsilonGreedy($\qapprox^{i}_p$, $s$)
            \STATE $s' \leftarrow$ EnvExecuteAction($s$, $a$)
            \FOR{$\qapprox^{o}_j \in \Qapprox$ \COMMENT{\textit{Learning loop}}}
                \STATE $u^{o}_k\leftarrow \delta^{o}_u(u^{o}_j,L(s'))$
                \STATE $r \leftarrow \delta^{o}_r(u^{o}_j,u^{o}_k)$
                \IF{EnvDeadEnd($s'$)} 
                    \STATE $\qapprox^{o}_j(s, a) \xleftarrow{\alpha} r(s,a,s') $
                \ELSE
                    \STATE $\qapprox^{o}_j(s, a) \xleftarrow{\alpha} r(s,a,s') + \gamma \max_{a'}{\qapprox^{o}_k(s', a')}$
                \ENDIF
            \ENDFOR
            \STATE $u^{i}_p \leftarrow \delta^{i}_u(u^{i}_p,L(s'))$; $s \leftarrow s'$
        \ENDFOR
        %\ENDWHILE
    \ENDFOR
\end{algorithmic}


==> src/qlearning.tex <==
\begin{algorithmic}[1]
    \STATE {\bfseries Input:} $S$, $A$, $\gamma \in (0,1]$, $\alpha \in (0,1]$, $\epsilon \in (0,1]$, $\mathcal{P}$, $L$, $U$, $u_0$, $F$, $\delta_u$, $\delta_r$.
    \STATE Initialize $\qapprox(s,u,a)$, for all $s \in S$, $u \in U$, and $a \in A$ arbitrarily
    \FOR{$l\leftarrow 0$ \TO num\_episodes} 
        \STATE Initialize $u \leftarrow u_0$ and $s \leftarrow$ EnvInitialState()
        \WHILE{$s$ is not terminal \AND $u \not\in F$} 
            \STATE Choose action $a$ from $(s,u)$ using policy derived from $\qapprox$ (e.g., $\epsilon$-greedy)
            \STATE Take action $a$ and observe the next state $s'$
            \STATE Compute the reward $r \leftarrow \delta_r(u)(s,a,s')$ and next RM state $u' \leftarrow \delta_u(u,L(s,a,s'))$
            \STATE Set experience $\leftarrow \{\tuple{s,u,a,r,s',u'}\}$
            \IF{Use counterfactual-experience}
                \STATE experience $\leftarrow \{\tuple{s,\bar{u},a,\delta_r(\bar{u})(s,a,s'),s',\delta_u(\bar{u},L(s,a,s'))} \ \ |\ \  \forall \bar{u} \in U\}$
            \ENDIF
            \FOR{$\tuple{s,\bar{u},a,\bar{r},s',\bar{u}'} \in $ experience}
                \IF{$s'$ is terminal \OR $\bar{u}' \in F$} 
                    \STATE $\qapprox(s,\bar{u},a) \xleftarrow{\alpha} \bar{r}$
                \ELSE
                    \STATE $\qapprox(s,\bar{u},a) \xleftarrow{\alpha} \bar{r} + \gamma \max_{a'\in A}{\qapprox(s',\bar{u}',a')}$
                \ENDIF
            \ENDFOR
            \STATE Update $s \leftarrow s'$ and $u \leftarrow u'$
        \ENDWHILE
    \ENDFOR
\end{algorithmic}

==> src/qrm.tex <==
\begin{algorithmic}[1]
    \STATE {\bfseries Input:} $S$, $A$, $\gamma \in (0,1]$, $\alpha \in (0,1]$, $\epsilon \in (0,1]$, $\mathcal{P}$, $L$, $U$, $u_0$, $F$, $\delta_u$, $\delta_r$.
    \STATE Initialize $\qapprox_u(s,a)$, for all $s \in S$, $u \in U$, and $a \in A$ arbitrarily
    \FOR{$l\leftarrow 0$ \TO num\_episodes} 
        \STATE Initialize $u \leftarrow u_0$ and $s \leftarrow$ EnvInitialState()
        \WHILE{$s$ is not terminal \AND $u \not\in F$} 
            \STATE Choose action $a$ from $s$ using policy derived from $\qapprox_u$ (e.g., $\epsilon$-greedy)
            \STATE Take action $a$ and observe the next state $s'$
            \FOR{$\bar{u} \in U$}
                \STATE Set $\bar{u}' \leftarrow \delta_u(\bar{u},L(s,a,s'))$
                \IF{$s'$ is terminal \OR $\bar{u}' \in F$} 
                    \STATE $\qapprox_{\bar{u}}(s,a) \xleftarrow{\alpha} \delta_r(\bar{u})(s,a,s')$
                \ELSE
                    \STATE $\qapprox_{\bar{u}}(s,a) \xleftarrow{\alpha} \delta_r(\bar{u})(s,a,s') + \gamma \max_{a'\in A}{\qapprox_{\bar{u}'}(s',a')}$
                \ENDIF
            \ENDFOR
            \STATE Update $s \leftarrow s'$ and $u \leftarrow \delta_u(u,L(s,a,s'))$
        \ENDWHILE
    \ENDFOR
\end{algorithmic}
